Wavelet-Based Fast Decoding of 360-Degree Videos

In this paper, we propose a wavelet-based video codec specifically designed for VR displays that enables real-time playback of high-resolution 360{\deg} videos. Our codec exploits the fact that only a fraction of the full 360{\deg} video frame is visible on the display at any time. To load and decode the video viewport-dependently in real time, we make use of the wavelet transform for intra- as well as inter-frame coding. Thereby, the relevant content is directly streamed from the drive, without the need to hold the entire frames in memory. With an average of 193 frames per second at 8192x8192-pixel full-frame resolution, the conducted evaluation demonstrates that our codec's decoding performance is up to 272% higher than that of the state-of-the-art video codecs H.265 and AV1 for typical VR displays. By means of a perceptual study, we further illustrate the necessity of high frame rates for a better VR experience. Finally, we demonstrate how our wavelet-based codec can also directly be used in conjunction with foveation for further performance increase.

==> sections/07_acknowledgments.tex <==
\section{Acknowledgments}

The authors gratefully acknowledge funding by the German Science Foundation (DFG MA2555/15-1 ``Immersive Digital Reality'').


